Visual-Thermal Landmarks and Inertial Fusion for Navigation in Degraded Visual Environments

With an ever-widening domain of aerial robotic applications, including many mission critical tasks such as disaster response operations, search and rescue missions and infrastructure inspections taking place in GPS-denied environments, the need for reliable autonomous operation of aerial robots has become crucial. Operating in GPS-denied areas aerial robots rely on a multitude of sensors to localize and navigate. Visible spectrum cameras are the most commonly used sensors due to their low cost and weight. However, in environments that are visually-degraded such as in conditions of poor illumination, low texture, or presence of obscurants including fog, smoke and dust, the reliability of visible light cameras deteriorates significantly. Nevertheless, maintaining reliable robot navigation in such conditions is essential. In contrast to visible light cameras, thermal cameras offer visibility in the infrared spectrum and can be used in a complementary manner with visible spectrum cameras for robot localization and navigation tasks, without paying the significant weight and power penalty typically associated with carrying other sensors. Exploiting this fact, in this work we present a multi-sensor fusion algorithm for reliable odometry estimation in GPS-denied and degraded visual environments. The proposed method utilizes information from both the visible and thermal spectra for landmark selection and prioritizes feature extraction from informative image regions based on a metric over spatial entropy. Furthermore, inertial sensing cues are integrated to improve the robustness of the odometry estimation process. To verify our solution, a set of challenging experiments were conducted inside a) an obscurant filed machine shop-like industrial environment, as well as b) a dark subterranean mine in the presence of heavy airborne dust.

==> 5Experimental_v2.tex <==
To evaluate the performance of our proposed algorithm, a set of experimental studies were conducted using an aerial robot in a) an indoor machine shop environment subject to the presence of dense fog and partial darkness, as well as b) a subterranean mine environment in the presence of heavy airborne dust. The robotic system used and the experiments conducted are detailed below.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h!]
\centering
  \includegraphics[width=0.99\columnwidth]{images/aeroconf_system_overview.eps}
\caption{The high-level processor, Intel NUC--i7, receives visual, thermal and inertial data from the Chameleon 3 camera, the Tau 2 thermal camera and the VN--100 IMU respectively in order to reliably estimate the robot pose. Furthermore, the high-level processor also receives inertial measurements from the autopilot of the robot and estimates smooth and robust robot odometry in real--time to enable state feedback position control.}
\label{fig:system}
\end{figure}



\subsection{System Overview}
For the purposes of experimental evaluation, a DJI Matrice 100 quadrotor equipped with the sensing suite proposed in this paper and an on-board computer was used. A FLIR Tau 2 thermal camera was mounted on the robot to provide thermal images of $640\times512$ resolution at $30$ frames per second. Two Pointgrey Chameleon 3 visible light CCD cameras, with shutter--synchronized LEDs, provided visual images of $644\times482$ resolution at $20$ frames per second. Only one of the visual cameras alongside the thermal camera was used during the experimental evaluations of this work. A VectorNav VN--100 IMU was employed to provide inertial measurements at an update rate of $200\textrm{Hz}$. The intrinsic calibration parameters of the visual and thermal cameras, as well the extrinsic calibration parameters for the IMU and the cameras were estimated using the work in~\cite{kalibr} and our custom designed thermal checkerboard pattern~\cite{ICUAS2018Thermal}. An Intel NUC--i7 computer (NUC7i7BNH) was carried on-board the robot to perform all high-level processing tasks. The estimated odometry from our proposed method is fused with inertial measurements received from the low--level attitude controlling autopilot of the robot using the the work of~\cite{msf}, in order to enable smooth and reliable position control using a Linear Model Predictive Control strategy based on the previous work of~\cite{mpc_rosbookchapter} for the robot. All algorithms were implemented as Robot Operating System (ROS) nodes and run in real-time fully on-board the robot. Figure~\ref{fig:system} provides the system overview of the robot system used.




%%

%\begin{minipage}{\textwidth}% to keep image and caption on one page
%\makebox[\linewidth]{%        to center the image
%  \includegraphics[keepaspectratio=true,scale=1]{images/maskvio_indoors_v2.eps}}
%\caption{A visualization of the robot trajectory during the indoor experiment. Inset a) shows the robot trajectory in green, b) shows an image of the robot during an instance of the experiment navigating from lit to dark parts of the environment, while c) and d) show images from the on-board visible and thermal cameras respectively at this instance during the robot trajectory.}
%\label{fig:indoors_rviz}%      only if needed  \end{minipage}
%\end{minipage}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Indoor Experiments}
To evaluate the real--time on-board performance of the proposed approach on an aerial robot, flight tests were conducted in an obscurant-filled environment. A fog generator was used to fill a machine shop resembling industrial environment with fog to serve as an obscurant during the experiment. Furthermore, lights were turned off in a section of the environment to simulate partial darkness and to demonstrate the robustness of our approach under varying lighting conditions and in the presence of obscurants during the same experiment. It should be noted that no on-board illumination was used in these experiments. The estimated robot trajectory during flight, from take--off to landing, is shown in  Figure~\ref{fig:indoors_rviz}.

%% INDOORS MAIN LARGE FIGURE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h!]
\centering
  \includegraphics[width=\columnwidth]{images/maskvio_indoors_v2.eps}
\caption{A visualization of the robot trajectory during the indoor experiment. Inset a) shows the robot trajectory in green, b) shows an image of the robot during an instance of the experiment navigating from lit to dark parts of the environment, while c) and d) show images from the on-board visible and thermal cameras respectively at this instance during the robot trajectory.}
\label{fig:indoors_rviz}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


To understand the effect of our feature selection approach on the track--ability of selected features inserted into the filter sate, we conducted 10 trials with and without using our feature selection region mask on the collected data-sets during the indoor experiments. The results of these trials are shown in Figure~\ref{fig:indoor_boxplot}. The plot demonstrates the benefit of our feature selection approach as the median number of features inserted in the filter state is smaller, indicating that the features selected using our proposed approach are tracked for a greater number of frames. Furthermore, to verify that our feature selection strategy provides a statistically significant difference in the selection of features we performed one--way Analysis of Variance (ANOVA) test on the population of features selected with and without the application of our approach. The test resulted in $p\text{-}value < 0.007185$, indicating that the two populations are statistically different from each other and verifies the effect of our proposed feature selection strategy.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h!]
\centering
  \includegraphics[width=0.99\columnwidth]{images/aeroconf_indoor_boxplot.eps}
\caption{Plot showing the total number of features inserted into the filter state, with and without the application of our proposed feature selection strategy, during the indoor experiments. Red line indicates the median value in each population, the blue box represents the interquartile range between the first and third quartiles and red $+$ symbols represent the outliers.}
\label{fig:indoor_boxplot}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Likewise, to understand the effect of our proposed feature selection strategy on the quality of the robot pose estimates, we analyze the evolution of the associated covariance of the robot pose estimates over time. As recommended in~\cite{dopt}, we employ the D-Optimality criterion as a metric for measuring uncertainty of our robot pose estimates. This takes the form:

\vspace{-2ex}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{eqnarray}\label{dopt}
D_{Optimality} = \exp(\log(\det(\Sigma)^{1/l}))
\end{eqnarray}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where $\Sigma$ is the robot pose covariance matrix with dimension $l$. The evolution of the D-Optimality criterion for the robot pose estimates over the length of the mission is shown in Figure~\ref{fig:indoor_dopt}. It can be noted that the application of our feature selection mask attenuates the accumulation of uncertainty in robot pose estimates, as features that can be tracked for more successive frames lead to better convergence of filter uncertainty estimates.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb]
\centering
  \includegraphics[width=0.99\columnwidth]{images/aeroconf_indoor_dopt.eps}
\caption{Plot showing the evolution of the robot pose uncertainty, using the D-Optimality criterion, with and without the application of our proposed feature selection strategy during an indoor experiment.}
\label{fig:indoor_dopt}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Subterranean Mine Experiment}
To demonstrate the real world performance and application of our approach, an experiment was conducted in a subterranean mine environment in conditions of darkness and heavy airborne dust. On-board illumination was utilized for vision cameras to function in the otherwise completely dark underground mine environment. To provide a measure ground truth markers were placed along the direction of the mine shaft with the final marker position being $50.0\textrm{m}$ away from the take-off position. The estimated robot trajectory during the experiment is shown in Figure~\ref{fig:mine_rviz}. A position error of $0.4857\textrm{m}$ was estimation along the direction of 



Similar to the analysis of indoor experiments, we conduct 10 trials on the collected data during the experiment to verify the effect of our approach. The respective plot is shown in Figure~\ref{fig:mine_boxplot}. As shown, the median number of features inserted into the filter state during the mission length using the proposed feature selection mask is lower as compared to not using it. Similarly, an ANOVA test was again performed on the two populations resulting in a $p\text{-}value < 0.00001$, validating that our approach makes a statistically significant difference on the selection of features to be used for estimation of odometry for the aerial robot.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h!]
\centering
  \includegraphics[width=0.99\columnwidth]{images/aeroconf_mine_boxplot.eps}
\caption{Plot showing the total number of features inserted into the filter state, with and without the application of our proposed feature selection strategy, during the subterranean mine experiments. Red line indicates the median value in each population, the blue box represents the interquartile range between the first and third quartiles and red $+$ symbols represent the outliers.}
\label{fig:mine_boxplot}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Similarly, Figure~\ref{fig:mine_dopt} shows the evolution of the pose uncertainty, using the D-Optimality criterion, over the trajectory of the aerial robot navigating through the subterranean mine environment. It is highlighted that the application of our feature selection mask results in a slowdown of the growth of pose uncertainty.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h!]
\centering
  \includegraphics[width=0.99\columnwidth]{images/aeroconf_mine_dopt.eps}
\caption{Plot showing the evolution of the robot pose uncertainty, using the D-Optimality criterion, with and without the application of our proposed feature selection strategy during a subterranean mine experiment.}
\label{fig:mine_dopt}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%% MINE MAIN LARGE FIGURE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[h!]
\centering
  \includegraphics[width=\textwidth]{images/maskvio_mine.eps}
\caption{A visualization of the robot trajectory as well as the position of pole markers placed to provide a measure of ground--truth during the subterranean mine experiment are shown in a), an image of the robot and the two observed pole markers during an instance of this experiment are shown in b), while c) and d) show the images captured from the on--board visual and thermal cameras respectively during an instance of the subterranean mine experiment.}
\label{fig:mine_rviz}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%show feature number
%big image showing 
